MATE: Multi-Attribute Table Extraction

A core operation in data discovery is to find joinable tables for a given table. Real-world tables include both unary and n-ary join keys. However, existing table discovery systems are optimized for unary joins and are ineffective and slow in the existence of n-ary keys. In this paper, we introduce MATE, a table discovery system that leverages a novel hash-based index that enables n-ary join discovery through a space-efficient super key. We design a filtering layer that uses a novel hash, XASH. This hash function encodes the syntactic features of all column values and aggregates them into a super key, which allows the system to efficiently prune tables with non-joinable rows. Our join discovery system is able to prune up to 1000x more false positives and leads to over 60x faster table discovery in comparison to state-of-the-art.

==> charts_and_tables/ICS.tex <==
\begin{table}[]
    \small
    \centering
    \caption{Initial query column selection experiment.}
    % \vspace{-.2cm}
    \label{tab:ICS}
\begin{tabular}{l|l|l|l|l|l}
&\textit{\textbf{Best}} & \textit{\textbf{\system}} & \textit{\textbf{Column Order}} & \textit{\textbf{TLS}} & \textit{\textbf{Worst}} \\ \toprule

AVG PL size & 83 & 179 & 202 & 246 & 728

\end{tabular}
\end{table}


==> charts_and_tables/kaggle_datasets.tex <==
\begin{table}[]
    \scriptsize
    \centering
    \caption*{Input Kaggle datasets.}
    % \vspace{-1em}
    \label{tab:datasets}
\begin{tabular}{l|l|l}
\toprule
\textit{\textbf{Dataset}} & \textit{\textbf{Query Columns (Composite key)}} & \textit{\textbf{Instances}} \\ \toprule
Pollution~\cite{kaggle_pollution}             & <State, City>       & 1,746,663\\ \hline
Open Food Facts~\cite{kaggle_food}             & <Product Name, brands>   & 356,000\\\hline
Wine~\cite{kaggle_wine}             & <Country, Province>    & 120,976        \\\hline
NYC Airbnb~\cite{kaggle_airbnb}             & <Neighbourhood Group, Neighbourhood>    & 48,000\\\hline
Cities~\cite{base_Cities}             & <Country, City>    & 40,000       \\ \hline%3173647       \\
Video Game Sales~\cite{kaggle_vgsales}             & <Name, Platform>  & 16,599 \\\hline
% PageView~\cite{base_pageview}          & <Name, Country>     & 11,000  \\\hline
Airline~\cite{kaggle_airline} & <Name, Country> & 6,163 \\\hline
Park~\cite{kaggle_park} & <Park, State> & 5,495 \\\hline
IMDB~\cite{base_imdb}& <Movie Title, Director Name> &  5,043  \\\hline
% Presidential~\cite{base_presidential}          & <State, County>            &  3,000\\\hline
Craft Beers~\cite{kaggle_beer}             & <Name, Style>         & 2,400\\\hline
Human Freedom Index~\cite{kaggle_hfi}             & <Country, Region> & 1,450\\\hline
% World Happiness Report~\cite{kaggle_happiness}             & <Country, Region>       & 157\\
% University~\cite{base_university}      & <Name, Location>        & 100  
\end{tabular}
\end{table}

==> charts_and_tables/variables.tex <==
% \begin{table}[]
%     \scriptsize
%     \centering
%     \caption{\answerRthree{List of variables used in the paper.}}
%     \label{tab:variables}
% \begin{tabular}{l|l}
% \toprule
% \textit{\textbf{Variable}} &
% \textbf{Description} \\ \toprule

% % $PL$ & Posting List that represents the location of a value in a table in corpus  \\
% % $m$ & The dimensionality of the join key  \\
% $\jmath$ & Joinability score  \\
% % $D$ & The input dataset\\
% % $Q$ & The set of columns in $D$ that form the composite key  \\
% % $T$ & Collection of tables that joinable tables are discovered from \\
% % $FP$ & False Positive  \\
% % $FN$ & False Negative  \\
% % $P$ & Number of all possible permutations\\
% % $c$ & The number of columns in a table\\
% % $v_i$ & Value i in the inverted index that maps to a list PL\\
% % $k$ & The number of joinable tables the system discovers \\
% $S_{ij}$ & The superkey of the $j^{th}$ PL of $v_i$\\
% $a$ & Bit array that contains the generated hash\\
% $L_{unique}$ & The number of unique values in the corpus\\
% $L_a$ & Hash size\\
% $\alpha$ & The optimum number of 1 bits in a\\
% $\beta$ & The number of bits in each character segment\\
% $L$ & The number of bits dedicated to the length segment\\
% $l_v$& Length of value v\\
% $\lambda$&Average location of the character to be hashed in the value\\
% $x$& Relative position of the character to be hashed in the value\\
% % $d$& Input dataset in the running example\\
% % $T_1$&Joinable table in the running example\\
% $\jmath_k$&Joinability score of the least joinable table among top-k discovered tables\\
% % $t$&Current candidate table to be evaluated\\
% $L_t$& The number of fetched PLs of table t\\
% $r_{checked}$&The number of evaluated rows from t\\
% $r_{matched}$&The number of row from t that are joinable to the input dataset\\
% % $h(k)$&hash result of key value k\\
% $q\textquotesingle$ & Query column with minimum cardinality\\
% \toprule
% \end{tabular}
% \end{table}





\begin{table}[]
    \scriptsize
    \centering
    \caption{\answerRthree{List of variables.}}
    \label{tab:variables}
\begin{tabular}{l|l}
\toprule
\textit{\textbf{Variable}} &
\textbf{Description} \\ \toprule
$\jmath$ & Joinability score  \\
$S_{ij}$ & The superkey of the $j^{th}$ PL of $v_i$\\
$a$ & Bit array that contains the generated hash\\
$C_{unique}$ & The number of unique values in the corpus\\
$|a|$ & Hash size\\
$\alpha$ & The optimum number of 1 bits in a\\
$\beta$ & The number of bits in each character segment\\
$|a_l|$ & The number of bits dedicated to the length segment\\
$l_v$& Length of value v, i.e., the number of characters in v\\
$\lambda$&Average location of the character to be hashed in the value\\
$x$& Relative position of the character to be hashed in the value\\
% $d$& Input dataset in the running example\\
% $T_1$&Joinable table in the running example\\
$\jmath_k$&Joinability score of the least joinable table among top-k discovered tables\\
% $t$&Current candidate table to be evaluated\\
$L_t$& The number of fetched PLs of table t\\
$r_{checked}$&The number of evaluated rows from t\\
$r_{matched}$&The number of row from t that are joinable to the input dataset\\
% $h(k)$&hash result of key value k\\
$q\textquotesingle$ & Query column with minimum cardinality\\
\toprule
\end{tabular}
\end{table}


==> sections/update_cache.tex <==
%!TEX root = ../main.tex

\section{Index Update }
There are three possible types of edits on table corpora that lead to updates in the index-level: {\em insert}, {\em update}, and {\em delete}.

Inserting a new table to the corpus requires the following updates.
Other than generating the PL items for the cell values in the newly added table, a super key is generated for each row. 
Inserting a new row to an existing table also follow the same procedure. 
Adding a new column to an existing table requires to apply \hash on each individual column value and replace the corresponding super key by the result of a bitwise-OR operation with the new \hash result.
Data updates also affect the super keys of affected tables.
For instance, updating the value of a cell requires a complete re-hash of the corresponding super key.
As the previous value is deleted, we cannot restrict the update to a bit-wise \texttt{OR} operation with the new hash value.
Deleting a table/row only requires deleting the PL items for the table/row.
Yet, deleting a column from a table might change the super key entries, triggering a rehashing of all rows.

Although some of the aforementioned updates require regeneration of the super key, the system can handle the changes locally to the affected table.
Generally, the most frequent index updates in a data lake would be \textit{table inserts}, which do not affect any of the already generated index values.

